Storing quantum information in spins and high-sensitivity ESR

Quantum information, encoded within the states of quantum systems, represents a novel and rich form of information which has inspired new types of computers and communications systems. Many diverse electron spin systems have been studied with a view to storing quantum information, including molecular radicals, point defects and impurities in inorganic systems, and quantum dots in semiconductor devices. In these systems, spin coherence times can exceed seconds, single spins can be addressed through electrical and optical methods, and new spin systems with advantageous properties continue to be identified. Spin ensembles strongly coupled to microwave resonators can, in principle, be used to store the coherent states of single microwave photons, enabling so-called microwave quantum memories. We discuss key requirements in realising such memories, including considerations for superconducting resonators whose frequency can be tuned onto resonance with the spins. Finally, progress towards microwave quantum memories and other developments in the field of superconducting quantum devices are being used to push the limits of sensitivity of inductively-detected electron spin resonance. The state-of-the-art currently stands at around 65 spins per root-Hz, with prospects to scale down to even fewer spins.

==> NecessaryPackages.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Geometry
\usepackage{mathptmx}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Images
\usepackage{graphicx} %images
\usepackage{graphics} %images
\usepackage{epstopdf}
\usepackage{pdfpages}
\graphicspath{{./Images/}} %repertoire des images

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Hyperref
%\usepackage{hyperref}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Others
\usepackage[english]{babel}
\usepackage{color}
\usepackage{amsmath, amsthm, amssymb}
\usepackage{bbold}
\usepackage{bm}
\usepackage{dsfont}
\usepackage{wrapfig} %text autour d'une image

